Smaller but Better: Self-Paced Knowledge Distillation for Lightweight yet Effective LCMs

Large code models (LCMs) have remarkably advanced the field of code generation. Despite their impressive capabilities, they still face practical deployment issues, such as high inference costs, limited accessibility of proprietary LCMs, and adaptability issues of ultra-large LCMs. These issues highlight the critical need for more accessible, lightweight yet effective LCMs. Knowledge distillation (KD) offers a promising solution, which transfers the programming capabilities of larger, advanced LCMs to smaller, less powerful LCMs. In this paper, we propose a novel Self-Paced knOwledge DistillAtion framework, named SODA, aiming at developing lightweight yet effective student LCMs. SODA consists of three stages in one cycle: (1) Correct-and-Fault Knowledge Delivery stage aims at improving the student models capability to recognize errors while ensuring its basic programming skill during the knowledge transferring, which involves correctness-aware supervised learning and fault-aware contrastive learning methods. (2) Multi-View Feedback stage aims at measuring the quality of results generated by the student model from two views, including model-based and static tool-based measurement, for identifying the difficult questions. (3) Feedback-based Knowledge Update stage aims at updating the student model adaptively by generating new questions at different difficulty levels, in which the difficulty levels are categorized based on the feedback in the second stage. Experimental results show that SODA improves the student model by 65.96% in terms of average Pass@1, outperforming the best baseline by 29.85%. Based on the SODA framework, we develop SodaCoder, a series of lightweight yet effective LCMs, which outperform 15 LCMs with less than or equal to 16B parameters. Notably, SodaCoder-DS-6.7B, built on DeepseekCoder-6.7B, even surpasses the prominent ChatGPT on average Pass@1.

==> Makefile <==
#
# Makefile for acmart package
#
# This file is in public domain
#
# $Id: Makefile,v 1.10 2016/04/14 21:55:57 boris Exp $
#

PACKAGE=acmart

DEV=-dev # To switch dev on
#DEV=

PDF = $(PACKAGE).pdf acmguide.pdf

BIBLATEXFILES= $(wildcard *.bbx) $(wildcard *.cbx) $(wildcard *.dbx) $(wildcard *.lbx)

SAMPLEBIBLATEXFILES=$(patsubst %,samples/%,$(BIBLATEXFILES))

ACMCPSAMPLES= \
	samples/sample-acmcp-Discussion.pdf \
	samples/sample-acmcp-Invited.pdf \
	samples/sample-acmcp-Position.pdf \
	samples/sample-acmcp-Research.pdf \
	samples/sample-acmcp-Review.pdf 

all:  ${PDF} ALLSAMPLES

%.pdf:  %.dtx   $(PACKAGE).cls
	pdflatex $<
	- bibtex $*
	pdflatex $<
	- makeindex -s gind.ist -o $*.ind $*.idx
	- makeindex -s gglo.ist -o $*.gls $*.glo
	pdflatex $<
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $*.log) \
	do pdflatex $<; done


acmguide.pdf: $(PACKAGE).dtx $(PACKAGE).cls
	pdflatex -jobname acmguide $(PACKAGE).dtx
	- bibtex acmguide
	pdflatex -jobname acmguide $(PACKAGE).dtx
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' acmguide.log) \
	do pdflatex -jobname acmguide $(PACKAGE).dtx; done

%.cls:   %.ins %.dtx
	pdflatex $<

%-tagged.cls:   %.ins %.dtx
	pdflatex $<


ALLSAMPLES: $(SAMPLEBIBLATEXFILES)
	cd samples; pdflatex samples.ins; cd ..
	for texfile in samples/*.tex; do \
		pdffile=$${texfile%.tex}.pdf; \
		${MAKE} $$pdffile; \
	done

samples/%: %
	cp $^ samples


samples/$(PACKAGE).cls: $(PACKAGE).cls
samples/$(PACKAGE)-tagged.cls: $(PACKAGE)-tagged.cls
samples/ACM-Reference-Format.bst: ACM-Reference-Format.bst

samples/abbrev.bib: ACM-Reference-Format.bst
	perl -pe 's/MACRO ({[^}]*}) *\n/MACRO \1/' ACM-Reference-Format.bst \
	| grep MACRO | sed 's/MACRO {/@STRING{/' \
	| sed 's/}  *{/ = /' > samples/abbrev.bib 


samples/%.bbx: %.bbx
samples/%.cbx: %.cbx
samples/%.dbx: %.dbx
samples/%.lbx: %.lbx



samples/%.pdf:  samples/%.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-biblatex.pdf: samples/sample-sigconf-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-acmsmall-biblatex.pdf: samples/sample-acmsmall-biblatex.tex $(SAMPLEBIBLATEXFILES)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	- cd $(dir $@) && biber $(notdir $(basename $<))
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	cd $(dir $@) && pdflatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && pdflatex${DEV} $(notdir $<); done

samples/sample-sigconf-xelatex.pdf:  samples/sample-xelatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	cd $(dir $@) && xelatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && xelatex${DEV} $(notdir $<); done

samples/sample-sigconf-lualatex.pdf:  samples/sample-lualatex.tex   samples/$(PACKAGE).cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	cd $(dir $@) && lualatex${DEV} $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex${DEV} $(notdir $<); done

samples/sample-acmcp.pdf: samples/acm-jdslogo.png


samples/sample-acmsmall-tagged.pdf:  samples/sample-acmsmall-tagged.tex   samples/$(PACKAGE)-tagged.cls samples/ACM-Reference-Format.bst
	cd $(dir $@) && lualatex-dev $(notdir $<)
	- cd $(dir $@) && bibtex $(notdir $(basename $<))
	cd $(dir $@) && lualatex-dev $(notdir $<)
	cd $(dir $@) && lualatex-dev $(notdir $<)
	while ( grep -q '^LaTeX Warning: Label(s) may have changed' $(basename $<).log) \
	  do cd $(dir $@) && lualatex-dev $(notdir $<); done



.PRECIOUS:  $(PACKAGE).cfg $(PACKAGE).cls $(PACKAGE)-tagged.cls

docclean:
	$(RM)  *.log *.aux \
	*.cfg *.glo *.idx *.toc \
	*.ilg *.ind *.out *.lof \
	*.lot *.bbl *.blg *.gls *.cut *.hd \
	*.dvi *.ps *.thm *.tgz *.zip *.rpi \
	samples/$(PACKAGE).cls \
	samples/$(PACKAGE)-tagged.cls \
	samples/ACM-Reference-Format.bst \
	samples/*.log samples/*.aux samples/*.out \
	samples/*.bbl samples/*.blg samples/*.cut samples/*.toc \
	samples/acm-jdslogo.png \
	samples/*.run.xml samples/*.bcf $(SAMPLEBIBLATEXFILES)


clean: docclean
	$(RM)  $(PACKAGE).cls $(PACKAGE)-tagged.cls \
	samples/*.tex

distclean: clean
	$(RM)  *.pdf samples/sample-*.pdf

#
# Archive for the distribution. Includes typeset documentation
#
archive:  all clean
	COPYFILE_DISABLE=1 tar -C .. -czvf ../$(PACKAGE).tgz --exclude '*~' --exclude '*.tgz' --exclude '*.zip'  --exclude CVS --exclude '.git*' $(PACKAGE); mv ../$(PACKAGE).tgz .

zip:  all clean
	zip -r  $(PACKAGE).zip * -x '*~' -x '*.tgz' -x '*.zip' -x CVS -x 'CVS/*'

# distros
distros: all docclean
	zip -r acm-distro.zip  \
	acmart.pdf acmguide.pdf samples *.cls ACM-Reference-Format.* \
	--exclude samples/sample-acmengage*
	zip -r acmengage-distro.zip samples/sample-acmengage* \
	samples/*.bib \
	acmart.pdf acmguide.pdf  *.cls ACM-Reference-Format.*

acmcp.zip: ${ACMCPSAMPLES} acmart.cls
	zip $@ $+

samples/sample-acmcp.tex: samples/samples.ins samples/samples.dtx
	cd samples; pdflatex samples.ins; cd ..


samples/sample-acmcp-%.tex: samples/sample-acmcp.tex samples/acm-jdslogo.png
	sed 's/acmArticleType{Review}/acmArticleType{$*}/' $< > $@

.PHONY: all ALLSAMPLES docclean clean distclean archive zip


==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

Version 2.12   Bug fixes
	       Switched to unicode-math and libertinus for Unicode engines

Version 2.11   Conference date is no longer printed in bibstrip.
	       ISBN now uses 4-digit year
	       DOI in bibliography is now output as doi:XX.XXXX/XXXXX.XXXX
	       Changed URL in Creative Commons licenses (deleted
	       trailing /legalcode)

Version 2.10.  Bug fixes.  Documentation update.

Version 2.09.  Experimental tagging code is now in the main branch.
	       Creative Commons license is now allowed for all materials. 

Version 2.08.  Section titles are in lowercase now.
	       Documentation updates.

Version 2.07.  Corrected typo in TELO eISSN.

Version 2.06.  Added eISSN for a number of journals.
               ACM no longer collects or prints authors'
	       postal addresses

Version 2.05   Changed title for TELO.

Version 2.04   Compatibility with the new latex-dev format
               eSSN is always printed, even if pSSN is present
	       Wording change in copyright statement

Version 2.03   Cleaned generation of samples.
	       New options for printing conference proceedings
	       in ACM journals

Version 2.02   Documentation update.
	       Changes in TOG templates
	       Corrected typo in ACM/IMS journals

Version 2.01   \acmPrice now produces a warning.

Version 2.00   ACM switches to electronic only version.
	       We do not print article tabs anymore.
	       New copyright wording.
	       Deleted \acmPrice.

Version 1.93   Added PACMSE

Version 1.92   Documentation update
	       Emergency change: changed order of hyperref and hyperxmp
	       due to changes in the undelying packages

Version 1.91   Minor changes in ACMCP format

Version 1.90a  Changes in the sample keywords and concepts

Version 1.90   Journal ISSN updated

Version 1.89a  Added version info to .bst

Version 1.89   Bug fixes
	       Redesign of ACMCP
	       New positioning of badges
	       New journals: PACMMOD, TOPML

Version 1.88   New ISSNs
	       Documentation updates
	       New journal:  PACMNET

Version 1.87   CC license is allowed for non-acm documents and ACM Engage
	       documents only
	       New format acmcp for the cover page
	       New journals: JATS, ACMJCSS, TORS
	       Bug fixes

Version 1.86.  Empty country in affiliation now produces an error
               Bug fixes
	       New samples for acmengage

Version 1.85.  Bug fixes
	       Added support for Creative Commons licenses (requires
	       doclicense images)
	       New journals
	       New format acmengage for ACM Engage CSEdu course materials 

Version 1.84   Support for BibLaTeX rewritten (thanks to
	       Roberto Di Cosmo and Kartik Singhal)
	       Corrected German translation (thanks to Dirk Beyer)
	       New journals

Version 1.83   Support for multilanguage papers
	       ISSN changes for some journals

Version 1.82   Bug fixes.
	       New command \anon for anonymization of short strings.
	       Documentation update.

Version 1.81   Bug fixes
	       New bib field distinctURL to print URL even if doi is present.
	       Reworded samples

Version 1.80   New journals: DLT, FAC

Version 1.79   Fixed pages with index
	       (https://github.com/borisveytsman/acmart/issues/440)
	       Updated information for TAP, TCPS, TEAC

Version 1.78   Documentation update.
	       Magic texcount comments for samples.
	       Title page now is split if there are too many authors
	       Bug fixes.

Version 1.77   Changed the way to typeset multiple affiliations (Christoph Sommer)

Version 1.76   Added many journal abbreviations to the bst.
	       New experimental option: pbalance
	       ORCID linking code

Version 1.75   Omitted \country now produces error.
	       Added \AtBeginMaketitle

Version 1.74   Bug fixes.  A regression introduced in the font changes
	       is reverted.

Version 1.73   Bug fixes
	       The elements institution, city and country are now obligatory
	       for affiliations.  The absence of them produces a warning

Version 1.72   Bug fixes.  Better handling of metadata.

Version 1.71   Bug fixes
               Formats sigchi and sigchi-a are retired
	       Bibliography formatting changes for @inproceedings entries
	       having both series and volume
	       LuaLaTeX now uses the same OTF fonts as XeLaTeX

Version 1.70   Title change for ACM/IMS Transactions on Data Science
               Bug fixes for bibliography

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.63a   Moved TQUANT to TQC

Version 1.63	New journals: TQUANT, FACMP

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.52    Another rewording of licenses

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.49    New jorunal:  DTRAP

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.47    New journal: THRI

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.43    Bug fixes

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.41    Rearranged bib files
                Added new badges

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.39    Added \authornotemark commmand

Version 1.38    Increase default font size for SIGPLAN

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

Version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

Version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

Version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

Version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

Version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

Version 1.28    Bug fixes: natbib=false now behaves correctly.

Version 1.27    Bug fixes

Version 1.26    Bug fixes

Version 1.25    Updated PACMPL journal option.

Version 1.24    Added IMWUT journal option.

Version 1.23    Added PACM PL journal option.

Version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

Version 1.21    Bibliography changes: added arXiv, some cleanup

Version 1.20    Bug fixes, documentation updates

Version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

Version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.


Version 1.17    Formatting changes for margins and lists.  Bug fixes.

Version 1.16    Formatting changes for headers and footers.

Version 1.15    New structured affiliation command.
                New commands for acknowledgements.

Version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

Version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

Version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

Version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

Version 1.10    Bug fixes

Version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

Version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes


==> datas/5.1.1_main_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \textcolor{red}{Don't waste too much time on here!}
% \begin{table*}[t]

% \renewcommand\arraystretch{1.15}
% \caption{Performance comparison of baseline methods.}
% \label{tab:comparison_main}
% \begin{tabular}{c|r|r|c|c|c|c|c|c|c|c}
% \toprule
% & \multicolumn{2}{r|}{} & \multicolumn{2}{c|}{Python} & Java     & JavaScript    &TypeScript   & C     &  C++       & Go      \\ \cline{4-11} 
% \multirow{-2}{*}{Model}  & \multicolumn{2}{r|}{\multirow{-2}{*}{Method}} & HumanEval   & MBPP   & MultiPL-E & MultiPL-E  & MultiPL-E & MultiPL-E & MultiPL-E & MultiPL-E \\ \midrule
%               & \multicolumn{2}{l|}{SFT}    &   &    &    &     &    &     &    &    \\
%               & \multicolumn{2}{l|}{RFT}     &     &    &    &    &    &    &    &    \\
%               & \multicolumn{2}{l|}{STAR}   &        &    &    &    &    &    &    &    \\
% \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}CodeLlama\\ -Base-7B\end{tabular}}   & \multicolumn{2}{c|}{$\text{ReST}^{\text{EM}}$}   &     &    &    &    &    &    &    &    \\ \midrule
% \rowcolor[HTML]{DADADA} \multicolumn{3}{c|}{\cellcolor[HTML]{DADADA}\tool-CL} &        &    &    &    &    &    &    &    \\ \midrule
%               & \multicolumn{2}{l|}{SFT}   &        &    &    &    &    &    &    &    \\
%               & \multicolumn{2}{l|}{RFT}   &        &    &    &    &    &    &    &    \\ 
%               & \multicolumn{2}{l|}{STAR}    &        &    &    &    &    &    &    &    \\ 
% \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}DeepSeek-Coder\\ -Base-7B\end{tabular}} & \multicolumn{2}{c|}{$\text{ReST}^{\text{EM}}$}  &  &    &    &    &    &    &    &    \\ \midrule
% \rowcolor[HTML]{DADADA} 
% \multicolumn{3}{c|}{\cellcolor[HTML]{DADADA}\tool-DS}  &    &    &    &    &    &    &    &   \\ \bottomrule    
% \end{tabular}
% \end{table*}


% \begin{table*}[t]
% % \small
% \caption{Performance comparison between {\tool} and baseline methods in terms of Pass@1.}
% \label{table:main}
% \begin{tabular}{c|cc|cccccc|c}
% \toprule
%  \multirow{2}{*}{Method}  & \multicolumn{2}{c|}{Python} & \multirow{2}{*}{Java} & \multirow{2}{*}{JS}  & \multirow{2}{*}{C}  &  \multirow{2}{*}{C++} & \multirow{2}{*}{Go} & \multirow{2}{*}{TS} & \multirow{2}{*}{Avg.}\\  \cline{2-3} 
%  & HumanEval   & MBPP    &  &   &   &  &  & & \\ \midrule
%  Base         & 35.4    & 46.8    & 35.9    &  32.9       &   25.1      & 29.2        &  30.4     & 32.0    & 33.4 \\\midrule
%   EVOL-INSTRUCT   & 48.7  & 50.0   & 55.4   &  52.4  & 41.7    & 39.6  & 43.2  &  50.0   &  47.6 \\
%   OSS-INSTRUCT   & 44.5  & 52.1   & 43.9    & 42.0  &  32.5  & 34.1   &  35.9   & 45.6  & 41.3 \\
%   PERsD  & 56.7    & 60.5   & 53.6   & 56.0    & 39.2   & 44.5   & 41.4  & 51.8   &  50.4\\ 
%   MFT  & 55.4   & 56.8   & 56.7   & 53.0    & 36.1   & 44.5   & 39.6  & 47.5   & 48.7 \\ \midrule
%  \tool   & \textbf{65.2}   & \textbf{65.3}   & \textbf{59.7}   & \textbf{58.5}  & \textbf{44.5}   & \textbf{46.9}   & \textbf{48.7}    & \textbf{55.5}  & \textbf{55.5} \\ \bottomrule 
% \end{tabular}
% \end{table*}

\begin{table*}[t]
% \small
\caption{Performance comparison between {\tool} and baseline methods in terms of Pass@1.}
\label{table:main}
\begin{tabular}{c|cc|cccccc|c}
\toprule
\multirow{2}{*}{Method} & \multicolumn{1}{c|}{HumanEval} & MBPP & \multicolumn{6}{c|}{MultiPL-E} & \multirow{2}{*}{Avg.} \\ \cline{2-9}
 & \multicolumn{2}{c|}{Python} & Java & JS & C & C++ & Go & TS &  \\ \midrule
Base & \multicolumn{1}{c|}{35.4 } & 46.8    & 35.9    &  32.9       &   25.1      & 29.2        &  30.4     & 32.0    & 33.4  \\\midrule
EVOL-INSTRUCT & \multicolumn{1}{c|}{48.7} & 50.0   & 55.4   &  52.4  & 41.7   & 39.6  & 43.2  &  50.0   &  47.6 \\
OSS-INSTRUCT & \multicolumn{1}{c|}{44.5} & 52.1   & 43.9    & 42.0  &  32.5  & 34.1   &  35.9   & 45.6  & 41.3  \\
PERsD & \multicolumn{1}{c|}{56.7 } & 60.5   & 53.6   & 56.0    & 39.2   & 44.5   & 41.4  & 51.8   &  50.4  \\
MFT & \multicolumn{1}{c|}{55.4 } & 56.8   & 56.7   & 53.0    & 36.1   & 44.5   & 39.6  & 47.5   & 48.7   \\\midrule
\textbf{\tool} & \multicolumn{1}{c|}{\textbf{65.2}}& \textbf{65.3}   & \textbf{59.7}   & \textbf{58.5}  & \textbf{44.5}   & \textbf{46.9}   & \textbf{48.7}    & \textbf{55.5}  & \textbf{55.5} \\ \bottomrule
\end{tabular}
\end{table*}

==> datas/5.1_main_table.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
% \usepackage[table,xcdraw]{xcolor}
% Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \textcolor{red}{Don't waste too much time on here!}
% \begin{table*}[t]

% \renewcommand\arraystretch{1.15}
% \caption{Performance comparison of baseline methods.}
% \label{tab:comparison_main}
% \begin{tabular}{c|r|r|c|c|c|c|c|c|c|c}
% \toprule
% & \multicolumn{2}{r|}{} & \multicolumn{2}{c|}{Python} & Java     & JavaScript    &TypeScript   & C     &  C++       & Go      \\ \cline{4-11} 
% \multirow{-2}{*}{Model}  & \multicolumn{2}{r|}{\multirow{-2}{*}{Method}} & HumanEval   & MBPP   & MultiPL-E & MultiPL-E  & MultiPL-E & MultiPL-E & MultiPL-E & MultiPL-E \\ \midrule
%               & \multicolumn{2}{l|}{SFT}    &   &    &    &     &    &     &    &    \\
%               & \multicolumn{2}{l|}{RFT}     &     &    &    &    &    &    &    &    \\
%               & \multicolumn{2}{l|}{STAR}   &        &    &    &    &    &    &    &    \\
% \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}CodeLlama\\ -Base-7B\end{tabular}}   & \multicolumn{2}{c|}{$\text{ReST}^{\text{EM}}$}   &     &    &    &    &    &    &    &    \\ \midrule
% \rowcolor[HTML]{DADADA} \multicolumn{3}{c|}{\cellcolor[HTML]{DADADA}\tool-CL} &        &    &    &    &    &    &    &    \\ \midrule
%               & \multicolumn{2}{l|}{SFT}   &        &    &    &    &    &    &    &    \\
%               & \multicolumn{2}{l|}{RFT}   &        &    &    &    &    &    &    &    \\ 
%               & \multicolumn{2}{l|}{STAR}    &        &    &    &    &    &    &    &    \\ 
% \multirow{-4}{*}{\begin{tabular}[c]{@{}c@{}}DeepSeek-Coder\\ -Base-7B\end{tabular}} & \multicolumn{2}{c|}{$\text{ReST}^{\text{EM}}$}  &  &    &    &    &    &    &    &    \\ \midrule
% \rowcolor[HTML]{DADADA} 
% \multicolumn{3}{c|}{\cellcolor[HTML]{DADADA}\tool-DS}  &    &    &    &    &    &    &    &   \\ \bottomrule    
% \end{tabular}
% \end{table*}


\begin{table*}[t]
\renewcommand\arraystretch{0.9}
% \renewcommand\arraystretch{1.15}
\caption{Performance comparison between {\tool} and baseline methods in terms of Pass@1.}
\label{table:main}
\begin{tabular}{c|cc|cccccc}
\toprule
 \multirow{2}{*}{Method}  & \multicolumn{2}{c|}{Python} & Java     & JavaScript    &TypeScript   & C  &  CPP   & Go \\ \cline{2-9} 
 & HumanEval   & MBPP    & MultiPL-E & MultiPL-E   & MultiPL-E  & MultiPL-E   & MultiPL-E   & MultiPL-E  \\ \midrule
 Base         & 35.4    & 46.8    & 35.9    &  32.9       & 32.0        &   25.1      & 29.2        &  30.4     \\\midrule
  SFT   & 48.7  & 50.0   & 55.4   &  52.4   &  50.0  & 41.7    & 39.6  & 43.2   \\
  RFT   & 50.0  & 55.5   & 57.9    & 50.0   & 50.6   &  40.4  & 40.1   &  45.1  \\
  STaR  & 54.9   & 58.7   & 59.1   & 53.0   & 48.7   & 36.8   & 42.6   & 45.1   \\ 
  $\text{ReST}^{EM}$  & 56.4    & 60.5   & 58.5   & 56.7   & 53.0   & 42.9   & 44.5   & 41.4   \\ \midrule
% \rowcolor[HTML]{DADADA} \tool & 65.2  & 63.3   & 59.7   & 58.5   & 55.5   & 44.2   & 46.9   & 48.7   \\ \bottomrule  
\rowcolor[HTML]{DADADA} \tool   & \textbf{65.2}   & \textbf{65.3}   & \textbf{59.7}   & \textbf{58.5}   & \textbf{55.5}   & \textbf{44.5}   & \textbf{46.9}   & \textbf{48.7}  \\ \bottomrule 
% \rowcolor[HTML]{DADADA} \tool-DS   & 67.1  &   &  68.9   & 58.5   &  64.1   & 51.5   & 58.5  &  53.0  \\ \bottomrule 
\end{tabular}
\end{table*}


==> datas/5.2.1_all_table.tex <==
\begin{table*}[t]
% \renewcommand*{\arraystretch}{1.15}
\caption{Pass@1 results of different LLMs/LCMs on HumanEval and MultiPL-E computed with greedy decoding. The abbreviations ``SC'', ``CL'' and ``DS'' refer to the student models StarCoder, CodeLlama and DeepseekCoder, respectively. We report the results consistently from the EvalPlus~\cite{EvalPlus} Leaderboard in August 2024. The cells in grey represent the performance of the top-3 best LCMs, with darker colors representing better performance. 
% Performance comparison between {\model} and various LLMs/LCMs in terms of Pass@1.
% We report the results consistently from the EvalPlus
% ~\cite{} Leaderboard.
}
\label{table:all_llm}
\footnotesize
\begin{tabular}{l|c|c|ccccccc|c}
\toprule
Model    & \begin{tabular}[c]{@{}c@{}}Release \\ Date\end{tabular} & Size & Python & Java & JS & C & C++ & Go & TS & Avg.\\ \midrule \midrule
\multicolumn{11}{c}{Proprietary Models}    \\ \midrule
GPT-4-turbo    & Apr 2024   & -      &  90.2      &  78.5    &  75.0     & 55.2    & 62.1      & 71.9 & 74.6   & 72.5 \\
ChatGPT   & Nov 2023   & -     &  76.8      &  64.2    &  61.1    & 44.5     &  57.3     & 62.2   & 63.4  & 61.3\\ \midrule \midrule
\multicolumn{11}{c}{Pre-trained Open-Source Models}      \\ \midrule
StarCoder      &  May 2023  &  15B     & 34.1     & 30.2     & 30.8         &  26.0   & 31.5   &  32.2  & 17.6   & 28.9 \\
CodeGen2       &  May 2023  &  16B     & 19.5       & 21.9     & 21.3         & 18.4    &  21.9     & 17.6   & 20.3   & 20.1 \\
CodeLlama  & Aug 2023    & 13B     & 42.7  &  42.6        & 37.1        &   32.5      &  32.9       &  33.5   & 43.2  & 37.7 \\ 
StarCoder2    & Feb 2024  &  15B     &  37.8     & 44.5        &  30.4            & 40.4        &  46.9       & 39.0    &   40.1  & 39.8 \\ \midrule
CodeLlama  & Aug 2023     &  7B     & 35.4  & 35.9    & 32.9       &   25.1       &  29.2   & 30.4   &  32.0    & 31.5 \\
DeepseekCoder   &  Nov 2023  &  6.7B   &  47.6   &  43.0    &    48.4       &  42.9   &  45.1   & 44.5   &   49.7   & 45.8 \\
StarCoder2   &  Feb 2024  & 7B      &  35.4      & 41.4   & 31.7           &  31.9       & 34.1        & 29.2  &   35.1   & 34.1 \\
CodeGemma &  Feb 2024    &  7B     &  48.4       &  48.4       & 46.0       & 42.2       &  41.4   & 34.2  & 48.7   &  44.1\\ 
CodeQwen1.5 & Apr 2024   & 7B      & 51.8       & 42.4     &  49.7    &  \colorbox{top3}{48.0} &  52.2   &  39.6  &  52.2  & 47.9 \\\midrule \midrule
\multicolumn{11}{c}{KD-based Open-Source Models}      \\ \midrule
WizardCoder-SC   & Jun 2023    &  15B  & 57.3   & 35.8     &   41.9    &  37.4   &  39.0    & 37.2  &  39.5    &  41.1   \\
MTFCoder-CL  & Nov 2023    & 13B     & 60.3  &  57.3     & 54.2     &  44.5      &  46.3    &  45.7  & 53.0  & 51.6 \\ \midrule
Magicoder-CL &  Dec 2023 &    7B     &   60.4      &  36.4    &   45.9   & 38.0    & 36.5  &  30.4  & 41.9      & 41.3 \\
Magicoder-DS   & Dec 2023  &   6.7B  &  \colorbox{top3}{66.5}   & 56.7     & 50.6   &   42.9     & \colorbox{top3}{53.6} &  50.6   & 52.4   & 53.3 \\
WaveCoder-DS & Apr 2024   &   6.7B   &  64.0   & \colorbox{top2}{64.0}    & 54.8   & 46.0   & 47.5    & \colorbox{top3}{53.6}    & \colorbox{top2}{56.1}   & \colorbox{top3}{ 55.1}\\
WaveCoderPro-DS & Apr 2024   &  6.7B   & \colorbox{top2}{72.0}   &  \colorbox{top3}{62.8}    &  \colorbox{top3}{57.9}   &  \colorbox{top2}{53.3}   &  \colorbox{top2}{56.0} & \colorbox{top2}{57.3}    & 54.9   &  \colorbox{top2}{59.1} \\ \midrule
\textbf{\model-CL} &  - &  7B  &  65.2   & 59.7   & \colorbox{top2}{\textbf{58.5}}  & 44.5  & 46.9   & 48.7 & \colorbox{top3}{\textbf{55.5}}  & 54.1 \\
\textbf{\model-DS} &  - &  6.7B & \colorbox{top1}{\textbf{74.3}}   & \colorbox{top1}{\textbf{73.1}}  &  \colorbox{top1}{\textbf{66.4}}    & \colorbox{top1}{\textbf{56.4}}  & \colorbox{top1}{\textbf{62.1}} &  \colorbox{top1}{\textbf{61.5}}  & \colorbox{top1}{\textbf{71.6}}  & \colorbox{top1}{\textbf{66.4}}\\ \bottomrule
\end{tabular}
\end{table*}

==> datas/5.2_all_table.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage[table,xcdraw]{xcolor}
% % Beamer presentation requires \usepackage{colortbl} instead of \usepackage[table,xcdraw]{xcolor}
% \begin{table*}[t]

% \renewcommand\arraystretch{1.15}
% \caption{Performance comparison of existing LLMs. We report the results consistently from the EvalPlus
% ~\cite{} Leaderboard.}
% \label{tab:comparison_all}

% \begin{tabular}{l|r|r|c|c|c|c|c|c|c|c}
% \toprule
% & \multicolumn{2}{r|}{} & \multicolumn{2}{c|}{Python}  & Java & JavaScript & C++ & PHP & Swift & Rust \\ \cline{4-11} 
% \multirow{-2}{*}{Model} & \multicolumn{2}{r|}{\multirow{-2}{*}{Size}} & HumanEval & MBPP & MultiPL-E & MultiPL-E & MultiPL-E & MultiPL-E & MultiPL-E & MultiPL-E \\ \midrule 
% \multicolumn{11}{c}{\cellcolor[HTML]{DADADA}Base Model}    \\
%                            & \multicolumn{2}{r|}{7B}      & 17.7   &       &      &       &     &     &       &      \\
% \multirow{-2}{*}{CodeGen2}  & \multicolumn{2}{r|}{16B}    &  16.5  &       &      &       &     &     &       &      \\ \midrule
%                             & \multicolumn{2}{r|}{7B}    &  29.9     &       &      &       &     &     &       &      \\
% \multirow{-2}{*}{StarCoder}  & \multicolumn{2}{r|}{15B}  &  37.8   &       &      &     &     &     &       &      \\ \midrule
%                              & \multicolumn{2}{r|}{7B}   & 35.4     & 46.8      &      &    &     &     &       &      \\
% \multirow{-2}{*}{CodeLlama}  & \multicolumn{2}{r|}{13B}  &   38.4     &  52.6  &      &    &     &     &     &   \\ \midrule
% CodeGemma    & \multicolumn{2}{r|}{7B}  &    41.5   &  52.4     &      &     &     &     &       &      \\ \midrule
% DeepSeek-Coder  & \multicolumn{2}{r|}{7B}   &  39.6    &  58.7     &      &            &     &     &       &      \\ \midrule
% \multicolumn{11}{c}{\cellcolor[HTML]{DADADA}Instrcution-tuned Model} \\
% \begin{tabular}[l]{@{}c@{}}CodeGen2.5\\ - instruct\end{tabular} & \multicolumn{2}{r|}{7B}                     &          &       &      &            &     &     &       &      \\ \midrule
% \begin{tabular}[l]{@{}c@{}}StarCoder2\\ - instruct\end{tabular}  & \multicolumn{2}{r|}{15B}  &  60.4 & 65.1     &      &            &     &     &       &      \\ \midrule
%                                  & \multicolumn{2}{r|}{7B}   &     &     &      &    &     &     &       &      \\
% \multirow{-2}{*}{\begin{tabular}[l]{@{}c@{}}CodeLlama\\ - instruct\end{tabular}}  & \multicolumn{2}{r|}{13B}  &       &   &      &    &     &     &     &   \\ \midrule
% \begin{tabular}[l]{@{}c@{}}CodeGemma\\ - instruct\end{tabular}  & \multicolumn{2}{r|}{7B} & 51.8  &  56.9      &      &            &     &     &       &      \\ \midrule
% \begin{tabular}[l]{@{}c@{}}DeepSeek-Coder\\ - instruct\end{tabular}  & \multicolumn{2}{r|}{7B}     &  71.3  &  62.2     &      &            &     &     &       &      \\ \midrule \midrule
% {\tool-CL}  & \multicolumn{2}{r|}{7B}   &       &       &      &            &     &     &       &      \\ 
% {\tool-DS}  & \multicolumn{2}{r|}{7B}   &       &       &      &            &     &     &       &      \\ 
% \bottomrule
% \end{tabular}

% \end{table*}


% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[t]
\renewcommand\arraystretch{0.9}
\caption{Performance comparison between {\model} and various LLMs/LCMs in terms of Pass@1.
% We report the results consistently from the EvalPlus
% ~\cite{} Leaderboard.
}
\label{table:all}
\begin{tabular}{l|r|cc|cccccc}
\toprule
\multirow{2}{*}{Model}   & \multirow{2}{*}{Size}  &  \multicolumn{2}{c|}{Python}   & Java     & JavaScript    &TypeScript   & C     &  CPP       & Go          \\ \cline{3-10}  
   &    & HumanEval  & MBPP  & MultiPL-E  & MultiPL-E   & MultiPL-E   & MultiPL-E    & MultiPL-E   & MultiPL-E       \\ \midrule
GPT-4 Turbo         & -             & 86.6    & 73.3    &  78.5    &  75.0       & 74.6       & 55.2    & 62.1      & 71.9        \\
GPT-3.5 Turbo     & 175B               & 70.7    & 69.7    &  64.2    &  61.1       & 63.4        & 44.5     &  57.3     & 62.2   \\
Llama-3  & 70B  & 76.8 &  72.0    &  71.3    &  62.8       & 66.0       & 58.5    & 58.9      & 60.9 \\ \midrule \midrule
\multicolumn{10}{c}{Over-30B-sized LCMs } \\ \midrule
CodeLlama          & 34B            & 43.9    & 56.3    &  39.6    &  45.4       & 44.5        & 31.2     &  40.1     & 34.7        \\
DeepSeek-Coder     & 33B            & 44.5    & 59.7   & 43.7     &  51.2       & 54.9        &   45.1      & 51.2     &  50.0       \\ \midrule \midrule
\multicolumn{10}{c}{Twice-sized LCMs } \\ \midrule
CodeGen2           & 16B            & 16.5    & 33.3    & 21.9     & 21.3     & 20.3     & 18.4    &  21.9     & 17.6        \\
StarCoder2         & 15B            & 37.8    & 55.5    & 44.5        &  30.4       &   40.1      & 40.4        &  46.9       & 39.0        \\
CodeLlama          & 13B            & 38.4    & 52.6    & 42.6        & 37.1        & 43.2        &   32.5      &  32.9       &  33.5       \\ \midrule \midrule
\multicolumn{10}{c}{Comparable-sized LCMs } \\ \midrule
CodeGen2           & 7B             & 17.7    & 34.3    & 25.0    &  17.6   &  20.3   & 15.3    &  18.2       & 16.4        \\
StarCoder2         & 7B             & 29.9    & 54.2    & 41.4   & 31.7     &   35.1      &  31.9       & 34.1        & 29.2        \\
CodeLlama          & 7B             & 35.4    & 46.8    & 35.9    &  32.9       & 32.0        &   25.1      & 29.2        &  30.4       \\
CodeGemma          & 7B             & 41.5    & 52.4    &  51.8       & 49.3        & 48.7        & 38.0        &  41.4       & 37.1        \\
DeepSeek-Coder     & 6.7B           & 39.6    & 58.7    &  56.0       &  45.7       & 50.6        &  42.9       &  45.1       & 44.5  \\ \midrule
\rowcolor[HTML]{DADADA} \model  & 7B   & \textbf{65.2}   & \textbf{65.3}   & \textbf{59.7}   & \textbf{58.5}   & \textbf{55.5}   & \textbf{44.5}   & \textbf{46.9}   & \textbf{48.7}  \\ \bottomrule
% \rowcolor[HTML]{DADADA} \model-DS  & 7B   & 67.1  &   &  68.9   & 58.5   &  64.1   & 51.5   & 58.5  &  53.0  \\ 

% \bottomrule
\end{tabular}

\end{table*}

==> datas/6.4_student.tex <==
\begin{table}[t]
% \setlength{\abovecaptionskip}{-0.01cm}
% \setlength{\belowcaptionskip}{-0.05cm}
\renewcommand\arraystretch{0.8}
\caption{Performance 
% comparison between the base and {\tool} methods 
of different student LCMs in terms of Pass@1.}
\label{table:student}
\begin{tabular}{c|c|cccc}
\toprule
Student          & Method                     & Python & Java & CPP & Go \\ \midrule
\multirow{2}{*}{CodeLlama-7B}        & Base     & 35.4  &  35.9    &  29.2   &  30.4  \\
                                     & {\tool} & \textbf{65.2}    &  \textbf{59.7}  & \textbf{46.9}    &  \textbf{48.7}   \\ \midrule
\multirow{2}{*}{DeepSeek-Coder-6.7B} & Base     & 39.6   & 56.0    & 45.1     &  44.5  \\
                                     & {\tool}  & \textbf{67.1}    &  \textbf{68.9}     &  \textbf{58.5}   &  \textbf{53.0}  \\ \bottomrule
\end{tabular}
\end{table}

==> sections/7_relatedWork.tex <==
\subsection{\modify{Large Code Models}} 

AI coding assistants are key applications of large language models (LLMs). Leading technology companies such as OpenAI and Google have developed proprietary models, such as GPT-4~\cite{} and Google Gemini~\cite{}, which show outstanding performance in coding tasks~\cite{}. On the other hand, specific LLMs pre-trained on extensive code corpus have been developed, such as 
Codex~\cite{}, AlphaCode~\cite{}, PanGuCoder~\cite{}, CodeLlama~\cite{}, DeepseekCoder~\cite{}, and CodeQwen~\cite{}. Apart from pre-training, instruction fine-tuning is also widely-used to further enhance the capabilities of LCMs, as showcased by WizardCoder~\cite{}, MFTCoder~\cite{}, Magicoder~\cite{}, and WaveCoder~\cite{}. Our model, {\model}, outperforms these by employing an adaptive knowledge distillation framework that continuously enhances its programming capabilities.

\subsection{\modify{LLMs for Code Generation}}

\modify{Iterative methods are commonly employed in sequence generation tasks to enhance output quality. For example, Self-Refine~\cite{} utilizes an LLM to iteratively refine initial outputs based on generated feedback. As for code generation, SELF-DEBUGGING~\cite{} teaches an LLM to debug its predicted program by examining execution results and providing explanations in natural language. Similarly, DebugBench~\cite{} shows that incorporating runtime feedback can improve the debugging performance of LLMs. Self-Edit~\cite{} trains a separate code editor to rectify generated code from the LLM. OpenCodeInterpreter~\cite{} integrates both execution results and human feedback for dynamic code refinement. Different from these approaches, our {\tool} framework uses multi-view feedback to categorize and update training data for iterative training, avoiding the need for costly output refinements during inference.
}





% Instruction tuning improves pre-trained LCMs by fine-tuning them with targeted instructions and corresponding responses. This technique adapts LCMs to handle specific tasks more effectively. 
% Wang~\etal utilize GPT-3 to generate synthetic instruction-response pairs with carefully crafted prompts for fine-tuning the same LLM~\cite{self-instruct}.
% Luo~\etal guide ChatGPT with heuristic prompts to produce complex synthetic data for fine-tuning StarCoder to obtain WizardCoder~\cite{WizardCoder}.
% Wei~\etal employ open-source code snippets to prompt LLMs generating instruction data for fine-tuning CodeLlama and DeepSeek-Coder to obtain Magicoder~\cite{Magicoder}. 
% %
% Different with these traditional instruction tuning methods, our framework incorporates dynamic data update and adaptive model refinement through iterative training cycles.

% \subsection{Data Augmentation}
% Data Augmentation (DA), in the context of LLMs, focuses on creating high-quality, task-specific datasets that are not only larger in volume but also rich in diversity and specificity.
% Wang~\etal introduce Self-Instruct~\cite{}, which leverages GPT-3 to generate synthetic instruction-response pairs with carefully crafted prompts. 
% Following this, Chaudhary~\etal apply Self-Instruct to ChatGPT, creating Code Alpaca~\cite{}, which includes 20,000 automatically generated code instructions. 
% Luo~\etal propose Code Evol-Instruct, guiding ChatGPT with heuristic prompts to produce more complex synthetic data. 
% Wei~\etal introduce OSS-Instruct, using open-source code snippets to prompt LLMs for generating instruction data. 
% Different from these static methods, our approach incorporates dynamic data augmentation during training, updating the data in response to the model's evolving programming capabilities.


% \subsection{Instruction Tuning}
% Instruction tuning improves pre-trained LCMs by fine-tuning them with targeted instructions and corresponding responses. This technique adapts LCMs to handle specific tasks more effectively. For example, DeepSeek-Coder-Instruct~\cite{} fine-tunes the basic DeepSeek-Coder based on 2 billion tokens of instruction data.
% CodeLlama-Instruct~\cite{} is fine-tuned based on an additional 5 billion tokens to enhance compliance with human instructions.
% WizardCoder~\cite{}, proposed by Luo~\etal, fine-tunes StarCoder using synthetic data generated by Code Evol-Instruct.
% Magicoder~\cite{}, proposed by Wei~\etal, is a family of models fine-tuned using OSS-Instruct.
% Different from these traditional instruction tuning methods, our approach not only ensures basic programming skills but also enhances error recognition abilities of models through iterative training cycles.


